Imitator Learning: Achieve Out-of-the-Box Imitation Ability in Variable Environments

Imitation learning (IL) enables agents to mimic expert behaviors. Most previous IL techniques focus on precisely imitating one policy through mass demonstrations. However, in many applications, what humans require is the ability to perform various tasks directly through a few demonstrations of corresponding tasks, where the agent would meet many unexpected changes when deployed. In this scenario, the agent is expected to not only imitate the demonstration but also adapt to unforeseen environmental changes. This motivates us to propose a new topic called imitator learning (ItorL), which aims to derive an imitator module that can on-the-fly reconstruct the imitation policies based on very limited expert demonstrations for different unseen tasks, without any extra adjustment. In this work, we focus on imitator learning based on only one expert demonstration. To solve ItorL, we propose Demo-Attention Actor-Critic (DAAC), which integrates IL into a reinforcement-learning paradigm that can regularize policies' behaviors in unexpected situations. Besides, for autonomous imitation policy building, we design a demonstration-based attention architecture for imitator policy that can effectively output imitated actions by adaptively tracing the suitable states in demonstrations. We develop a new navigation benchmark and a robot environment for \topic~and show that DAAC~outperforms previous imitation methods \textit{with large margins} both on seen and unseen tasks.

==> main-4-method-1-imitator-reward.tex <==

\cite{ciosek2021imitation} has shown that, for deterministic experts, IL can be done by RL with a constructed stationary reward.  Inspired by this, we propose to construct a stationary imitator reward $R_{Itor}$ to embed IL into the RL process,  i.e., replacing the reward function $R_\omega$ in Alg.~\ref{alg:framework}(Line 7) with $R_{Itor}$. $R_{Itor}$ is heuristic designed based on our observations on the limitations of the imitation rewards proposed by \cite{ciosek2021imitation} in imitator learning scenarios. We leave the full discussion in Appendix\ref{app:imitation_reward}. To handle the above problems, we construct a new imitator reward function $\rewfunc_{\rm Itor}(s,a)$ via:






\begin{equation}
    \label{eq:reward}
	1 - \min\Big{\{}d(\bar s, s)^2 + \frac{d(\bar a, a)^2}{\exp(d(\bar s, s)^2)},  \eta\Big{\}}  + \alpha R_{\mparam}(s,a),
\end{equation}
where $(\bar s, \bar a) = \arg \min_{(s',a')\in \demoset} d(s,s')^2$. 
The selected action $\bar a$ corresponds to the action associated with state $\bar s$ in the transition pair. $\eta$ is a hyperparameter that clips the distance penalty calculated based on the too-far state pairs into a fixed constant, $\alpha = 1/(\finalrew(1-\discount))$ is a rescale coefficient, and $\finalrew$ is the reward for accomplishing the task defined in $R_{\mparam}$. \yejy{Note that the term $d(\bar s, s)$ measures the distance between $\bar s$ and $s$, and it can be customized differently for different tasks. In this work, we adopt L2 distance.}

\yejy{The core motivation of the $R_{Itor}(s,a)$ design is to guide policy learning efficiently across multiple tasks by combining imitation reward $R_{IL}$ and ending reward $R_{\mparam}$. During the early stages of learning, $R_{IL}$ serves as a crucial signal by providing a dense reward, enabling the agent to closely follow the demonstrations and accomplish tasks effectively. However, relying solely on $R_{IL}$ may lead to ill-posedness issues. Hence, the ending reward is essential, as it helps the agent focus more on task completion rather than repeatedly collecting $R_{IL}$ rewards. By leveraging the training process of RL, our algorithm optimizes based on the demonstrations, facilitating faster task completion.}

$R_{\rm Itor}(s,a)$ uses \yejy{\textbf{a clipping term}} $\eta$ to make the imitation rewards based on the too-far state pairs invalidated to avoid the potential misleading (to handle the ``$A$-state'' case). \yejy{\textbf{A reweighting item}} $1/\exp(d(\bar s, s)^2)$ is used for action's distance computation adaptively adjusts the weight of rewards on action matching. This is a heuristic reweighting term to avoid the agent overly penalizing for not strictly following the expert action when its current state is far from the demonstration states and chooses to turn back  (to handle the ``$B$-state'' case). \yejy{The necessity of the reweighting term stems from its pivotal role in preventing undesired behaviors in situations where the agent strictly adheres to the demonstrated actions due to state bias. By incorporating the reweighting term, we ensure that the agent does not blindly follow the demonstrations, thereby reducing the risk of unintended consequences.}
$\alpha$ rescales the ending rewards, which makes the discount on delay to get the ending reward larger than the bonus of repeatedly collecting the immediate rewards, i.e., $\alpha \finalrew > 1 - \epsilon + \gamma \alpha \finalrew$, where $\epsilon$ denotes a larger-than-zero penalty contributed by the second item in Eq.~\ref{eq:reward} (to handle the ``$C$-state'' case). \yejy{Lastly, we opted for a linear combination for its simplicity and ease of controlling the dominance of ending reward numerically through reweighting. 
}
Note that we do not analyze the theoretical property of $R_{\rm Itor}$. Similar to $\rewfunc_{\rm IL}$ in \cite{ciosek2021imitation}, we verify it in practice. We leave the theoretical analysis as future work.

\yejy{
    The reward function $R_{\rm Itor}(s,a)$ is designed heuristically and may have ill-posed corner cases. 
    It may reduce to $1 - \eta  + \alpha R_{\mparam}(s,a)$ when  $d(\bar s, s)$ is too large. In this case,  $R_{\mparam}(s,a)$ is sparse and harm the exploration. 
    However, we would like to emphasize that in our study, this issue is not particularly severe. By our definition, different tasks share the same initial state distribution, and under this initial state distribution, there exists a retrievable $\beta$ policy from a single demonstration. This requires that the distribution of the initial state is not too diverse, otherwise, there wouldn't be a unified $\beta$ policy that can be traced back to the demonstration. Hence, 
    at the starting state, the problem of sparse rewards, is unlikely to occur. This makes it relatively easier for the policy to follow the demonstration step-by-step until the objective is achieved. We will verify this in Sec.~\ref{sec:far_away} by conducting an experiment that increase the scale of the randomness in initial state distribution. 
    }




==> main-4-method-3-schedule.tex <==



==> nips_math_command.tex <==
\newcommand{\topic}{ItorL}
\newcommand{\algo}{DAAC}



\newcommand{\tv}{D_{\rm TV}}
\newcommand{\kl}{D_{\rm KL}}
\newcommand{\dataset}{\mathcal{D}}
\newcommand{\mdp}{\mathcal{M}}

\newcommand{\sspac}{\mathcal{S}}
\newcommand{\aspac}{\mathcal{A}}
\newcommand{\discount}{\gamma}
\newcommand{\traj}{\tau}
\newcommand{\horizon}{H}
\newcommand{\acs}{a}
\newcommand{\state}{s}
\newcommand{\rew}{r}
\newcommand{\rewfunc}{R}
\newcommand{\trans}{T}
\newcommand{\ts}{i}
\newcommand{\initdist}{d_0}
\newcommand{\perf}{J}

\newcommand{\buffer}{\mathcal{B}}
\newcommand{\piparam}{\theta}
\newcommand{\mparam}{\omega}
\newcommand{\mparamspac}{\Omega}
\newcommand{\qparam}{\psi}

\NewDocumentCommand{\vpim}{O{\pi} O{}}{V^{#1}_{#2}}
\NewDocumentCommand{\qpi}{O{\pi}}{Q^{#1}}
\NewDocumentCommand{\occ}{O{\pi} O{\state_0}}{\rho^{#1}_{#2}}


\NewDocumentCommand{\transF}{O{\state} O{\acs} O{\state'}}{\trans({#3}| {#1}, {#2})}
\NewDocumentCommand{\rewF}{O{\acs} O{\state}}{\rewfunc({#1}, {#2})}
\NewDocumentCommand{\piF}{O{}  O{\state} O{\acs}}{\pi_{#1}({#3}|{#2})}
\NewDocumentCommand{\vF}{ O{\pi} O{} O{\state}}{\vpim[#1]{#2}({#3})}
\NewDocumentCommand{\qF}{O{} O{\pi} O{\state}  O{\acs}}{\qpi[#2]_{#1}({#3, #4})}

\NewDocumentCommand{\occdist}{O{\pi}}{\occ[#1][\initdist]}

\newcommand{\demoset}{\mathcal{T}}
\newcommand{\mdpset}{\mathbb{M}}
\newcommand{\extract}{\phi}
\newcommand{\hid}{z}
\newcommand{\hidspac}{\mathcal{Z}}
\newcommand{\finalrew}{c}



==> related_work.tex <==
\section{Related work}

\subsection{Imitation Learning}



IL focuses on training a policy with action labels from expert demonstrations. 
There are two mainstream approaches for IL, namely behavior cloning (BC)~\citep{bc1, BC} and inverse reinforcement learning (IRL)~\citep{IRL}. 
The former BC converts imitation learning into a supervised paradigm by minimizing the action probability discrepancy with Kullback–Leibler (KL) divergence between the actions of the imitating policy and the demonstration actions.  The latter IRL fashion learns the hidden reward function behind the expert policy to avoid the impact of compounding errors.
Since IL can learn directly from already collected data, it is widely adopted by complex domains like game playing~\cite{RossB10}, autonomous driving~\citep{PanCSLYTB18, ChenYT19}, and robot manipulation~\citep{0005CKZWY20}.  Although achieving impressive performances,  we observe that in many applications, what humans require is the ability to perform many different tasks out of the box, through very limited demonstrations of corresponding tasks, instead of imitating from scratch based on a mass of demonstrations. 
Adapting the trained policy to unseen tasks is beyond the capability of pure IL, which is designed for single task learning.



Few-Shot Imitation Learning aims to get a generalizable policy that can complete new tasks with only a few expert trajectories. 
The mainstream solutions utilize model-agnostic meta-learning (MAML)~\citep{finn2017model} to learn initial task parameters and fine-tune them via a few steps of gradient descent to satisfy new task needs~\citep{MIL,yu2018one,li2021meta}.  However, these approaches need extra computation infrastructure for gradient update and determining a suitable amount of fine-tuning steps before being deployed \citep{finn2017model}.
Other methods achieve generalizable imitation through context-based policy models~\cite{duan2017one, dasari2021transformers, mandi2022towards}, such as Transformer~\citep{transformer}, that take demonstrations as input. 
The core idea is to extract representations of demonstrations through thes powerful fitting ability of neural networks, then use BC to reconstruct the imitation policy. 
However, the demonstrations for imitation are limited, the inevitable prediction errors on unseen states and the compounding errors of BC~\citep{dagger} hurt the capacities of these methods, especially in generalizing to new tasks~\citep{mandi2022towards}.
Our ItorL method also utilizes a context-based model to achieve the out-of-the-box imitation ability. Instead of using BC, we inject IL into the RL process, which allows the agent to interact with the environment. This approach can regularize the policy behavior facing states unseen in demonstrations.



We are not the first study to combine IL and RL. Previous studies have combined these for different proposes:
\citet{HesterVPLSPHQSO18} leverage small sets of demonstrations for deep q-learning which massively accelerates the learning process. \citet{rajeswaran2017learning} use demonstrations to reduce the sample complexity of learning dexterous manipulation policy and enable natural and robust robot movement.
\citet{FujimotoG21} add BC to the online RL algorithm TD3~\citep{fujimoto2018addressing} for advanced offline RL performance. 
Our method extends the ideas of combining IL and RL to handle a new problem: a multi-policy imitation problem based on limited demonstrations.




\subsection{Context-based Meta Reinforcement Learning}

Besides IL,  context-based policy models are also widely used in meta RL.  
Building a representative context  enables a single agent of learning meta-skills and identifying new tasks. Goal-conditioned RL \citep{FlorensaHGA18, NairSF20} is the most direct way to build a context-based meta policy, which scales a single agent to a diverse set of tasks by informing the agent of the explicit goal contexts, e.g., the target to go or the object to pick.
The demonstrations can be regarded as an informative ``goal'' for IL tasks. The demonstration sequence not only tells the agent which task to accomplish but the way to accomplish the task.

Some other works collect interaction trajectories from the environment for understanding the task identity. \cite{osi-lstm,cube_adr,learn_to_adapt,maple,luo2022adapt} use a end-to-end architecture for environment-parameter representation and adaptable policy learning. A recurrent neural network is introduced for environment-parameter representation, then the context-aware policy takes actions based on the outputs of RNN and the current states.  \cite{pearl} share the same end-to-end architecture and design a new neural network to represent the probabilistic latent contexts of the environment parameters.
Instead of collecting trajectories from the environment for identifying the task, we mine the information from the static expert trajectories to identify the expert policy which can accomplish the task. 

Demonstration-conditioned RL (DCRL)~\cite{dcrl} takes suboptimal demonstrations as input and seeks to further improve demonstration behavior via RL. ~\citet{YehCSCH22} adopt a similar idea to solve unseen compound robot tasks that contain multiple stages by retrieving from demonstrations.  
Instead of taking demonstration as the base for policy improvement, ItorL aims to fully utilize the demonstrations to imitate the expert policy for each task.


















